A Comprehensive Survey of Advanced Persistent Threat Attribution: Taxonomy, Methods, Challenges and Open Research Problems

Advanced Persistent Threat (APT) attribution is a critical challenge in cybersecurity and implies the process of accurately identifying the perpetrators behind sophisticated cyber attacks. It can significantly enhance defense mechanisms and inform strategic responses. With the growing prominence of artificial intelligence (AI) and machine learning (ML) techniques, researchers are increasingly focused on developing automated solutions to link cyber threats to responsible actors, moving away from traditional manual methods. Previous literature on automated threat attribution lacks a systematic review of automated methods and relevant artifacts that can aid in the attribution process. To address these gaps and provide context on the current state of threat attribution, we present a comprehensive survey of automated APT attribution. The presented survey starts with understanding the dispersed artifacts and provides a comprehensive taxonomy of the artifacts that aid in attribution. We comprehensively review and present the classification of the available attribution datasets and current automated APT attribution methods. Further, we raise critical comments on current literature methods, discuss challenges in automated attribution, and direct toward open research problems. This survey reveals significant opportunities for future research in APT attribution to address current gaps and challenges. By identifying strengths and limitations in current practices, this survey provides a foundation for future research and development in automated, reliable, and actionable APT attribution methods.

==> Section/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The threat attribution process focuses to distinguish the operational behaviour, attack patterns of threat actors~\cite{steffens2020attribution}\fix{apt threat profiling survey}.
The malware-based threat attribution methods present in the literature leverage various features like words of cuckoo sandbox report, opcodes, bytecodes, API calls, Header data, Intermediate Representation of executable, string features, fuzzy hashes, and CFGs. Methods based on words of cuckoo sandbox reports focuses 

~\ref{tab:methodperformancecomp}.


The papers discussed exhibit a variety of strengths and weaknesses in their approach to threat attribution. Malware-based analyses benefit from detailed behavioral insights but often face challenges in computational demands and scalability. Threat report-based methods offer practical insights but can struggle with generalizability and data dependency. Attack pattern-based methods effectively focus on TTPs but may suffer from high dimensionality and complexity in feature management. Heterogeneous data-based approaches provide a comprehensive view but face significant challenges in data integration and scalability. Each method has its unique contributions and limitations, which should be considered in the context of specific threat attribution needs and environments.

% \begin{table*}[]
%     \centering
%     \caption{Attribution Method Performance Comparison}
%     \label{tab:methodperformancecomp}
%     \input{Table/PerformanceComparison}
% \end{table*}

==> Section/Lesson_Learned.tex <==
\section{Lesson Learned}
\label{sec:lessonlearned}

The survey reveals several key insights that are crucial for the field of cyber threat attribution. Integrating various intelligence sources, including OSINT and dark web data, alongside traditional CTI, is essential for a comprehensive understanding of threat actors. Advanced honeypots and deception techniques, particularly those enhanced with AI, prove valuable in capturing and analyzing attack data with minimal human intervention, enabling more accurate attribution.

Developing sophisticated attribution algorithms, such as those using GNNs and context-aware methods, significantly enhances the precision and efficiency of attribution efforts. Cross-disciplinary collaboration enriches the technical data with contextual insights from cybersecurity, geopolitics, sociology, and intelligence analysis, leading to more robust conclusions.

The robustness of attribution models against coordinated and adversarial attacks is vital. Advanced anonymization techniques and false flags used by APT groups require resilient models and continuous learning mechanisms to adapt to the evolving threat landscape.

Ethical and privacy considerations are paramount, necessitating privacy-preserving techniques and ethical guidelines to ensure responsible use of attribution technologies. Lastly, standardized benchmarking datasets and evaluation metrics are crucial for rigorous assessment, driving continuous improvement and ensuring the reliability and accuracy of attribution methods. These lessons provide a solid foundation for advancing research and practical applications in cyber threat attribution.

==> Table/MethodComparison.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Comparison of Attribution Methods}
    % \input{tables/APTMethodComparison}
    \label{tab:aptmethodcomp}
    % \begin{tabularx}{\textwidth}{|p{1.5cm}|p{0.8cm}|p{1.3cm}|p{1.3cm}|p{2cm}|p{1.3cm}|p{1cm}|p{1cm}|p{0.8cm}|p{1.2cm}|X|}
    \begin{tabularx}{\textwidth}{|p{0.5cm}|p{0.7cm}|p{1.5cm}|X|X|X|p{1cm}|p{1cm}|p{0.8cm}|p{1.2cm}|p{1.3cm}|}
     \hline
    \multirow{2}{*}{\textbf{Paper}} & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Feature}} & \textbf{Feature} & \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{4}{|c|}{\textbf{Reported Performance}} & \textbf{Code}\\
    \cline{7-10}
    & &  & & \textbf{Vector} & & \textbf{Accuracy (\%)}   & \textbf{Precision (\%)}   & \textbf{Recall (\%)}   & \textbf{F1-score (\%)} & \textbf{Availability} \\
    \hline
    \hline
    ~\cite{rosenberg2017deepapt} & $2017$ & Malware-based & Cuckoo sandbox reports & One-Hot encoding of report words & DNN & $94.6$ & $-$ & $-$ & $-$ & \\
    \hline
    ~\cite{perry2019no} & $2019$ & Threat Report-based & Report words & SMOBI Word Embeddings & XGBoost & $58.4$ & $55$ & $52.4$ & $-$ & \\
    \hline
    ~\cite{noor2019machine} & $2019$ & Attack Pattern-based & TTPs & One-Hot encoding  & DNN & $94$ & $90$ & $89$ & $89$  & \\
    \hline
    ~\cite{haddadpajouh2020mvfcc} & $2020$ & Malware based & OpeCode, ByteCode, System call, and Header & OH, Count, TF-IDF, Eigen Vector and Frequency of Occurrence & DT &  $95$ & $-$ & $-$ & $-$ & \\
    \hline
    ~\cite{wu2020grouptracer} & $2020$ & Attack Pattern-based & Time, IP, URL, and TTPs mapped from IoT honeypot logs & Statistical characteristics for each feature types & Hierarchical clustering &  &  &  &  &  \\
    \hline
    ~\cite{naveen2020deep} & $2020$ & Threat Report & Report words & SIMVER Word Embeddings & DNN & $86.5$ & $95.4$ & $83.3$ & $87.9$ & \\
    \hline
    ~\cite{xu2021apt} & $2021$ & Malware & API call sequence & n-gram with Adaboost feature selection & DT, KNN, LightGBM, and XGBoost & $93.53$ & $89.65$ & $84.72$ & $86.62$  &  \\
    \hline
    ~\cite{wang2021explainable} & $2021$ & Threat Report and Malware & IR code and string features & Paragraph and bag-of-words vectors & RF and DNN & $97.87$ & $-$ & $-$ & $-$  &  \\
    \hline
    ~\cite{li2021attribution} & $2021$ & Malware & Cuckoo sandbox behaviour reports & TF-IDF with Chi-square for dimensionality reduction & SMOTE and RF & $-$ & $85$ & $79.1$ & $79.4$  &  \\
    \hline
    ~\cite{kim2021automatically} & $2021$ & Attack Pattern-based & TTPs & Tactics-wise One-Hot encoding & k-means clustering & $-$ & $91.48$ & $95.14$ & $93.27$ &   \\
    \hline
    ~\cite{shin2021art} & $2021$ & Attack Pattern-based & TTPs  & Tactics-wise One-Hot encoding & Cosine similarity with weighted tactic vectors & $-$ & $-$ & $-$ & $-$  & \\
    \hline
    ~\cite{kida2022nation} & $2022$ & Malware & Fuzzy hashes (TLSH, SSDEEP, SDHASH, IMPFUZZY, and  LZJD) & NATO Encoding & RF, SVM, KNN, and NB & $89$ & $-$ & $-$  & $88$ &  \\
    \hline
    ~\cite{wang2022apt} & $2022$ & Malware & Control Flow Graph (CFG) & Basic blocks characteristics with PCA fro dimensionality reduction & HDBSCAN clustering &  &  &  &  &  \\
    \hline
    ~\cite{lee2022malware} & $2022$ & Malware & Runtime Modules like Kernel32.dll &  Frequency analysis and  One-Hot  encoding & KNN, SVM, DT, NB, Adaptive and Gradient Boosting) & $93.5$ & $88$ & $87$ & $87$ & \\
    \hline
    ~\cite{mei2022hybrid} & $2022$ & Heterogeneous Data-based  & Traces field values & TF-IDF & Multi-class SVM with Particle Swarm Optimization  & $93.96$  & $93.97$  &  & $93.94$ &   \\
    \hline
    ~\cite{xu2022hghan} & $2022$ & Heterogeneous Data-based  &Web attack heterogeneous graphs  & Node embedding & BiLSTM  & $98$ & $97$ & $98$ &  $97$ &   \\
    \hline
     ~\cite{edie2023extending} & $2023$ &  Attack Pattern-based & MITRE TTP and it's association  & TTP List & Wighted Jaccard Index & 95.7 & $-$ & $-$ & $-$ & Yes  \\
    \hline
    ~\cite{noor2023machine} & $2023$ & Heterogeneous Data-based  & TTPs and Softwares used & One-Hot & Neural Network & $94.88$ & $93.95$ & $94.88$ & $94$  &   \\
    \hline
    \multicolumn{11}{>{\footnotesize\itshape}r}{Continue on the next page}
\end{tabularx}
    \end{table*}


\begin{table*}[!ht]
    \ContinuedFloat
    \centering
    \caption{Comparison of Attribution Methods}
    % \begin{tabularx}{\textwidth}{|p{1.5cm}|p{0.8cm}|p{1.6cm}|p{1.3cm}|p{1.7cm}|p{1.3cm}|p{1cm}|p{1cm}|p{0.8cm}|p{1.2cm}|X|}
    \begin{tabularx}{\textwidth}{|p{0.5cm}|p{0.7cm}|p{1.5cm}|X|X|X|p{1cm}|p{1cm}|p{0.8cm}|p{1.2cm}|p{1.3cm}|}
     \hline
    \multirow{2}{*}{\textbf{Paper}} & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Type}} & \multirow{2}{*}{\textbf{Feature}} & \textbf{Feature} & \multirow{2}{*}{\textbf{Algorithm}} & \multicolumn{4}{|c|}{\textbf{Reported Performance}} & \textbf{Code}\\
    \cline{7-10}
    & &  & & \textbf{Vector} & & \textbf{Accuracy (\%)}   & \textbf{Precision (\%)}   & \textbf{Recall (\%)}   & \textbf{F1-score (\%)} & \textbf{Availability} \\
    \hline
    \hline
    % Ren et. al~\cite{ren2022cskg4apt} & $2022$ & Heterogeneous Data-based  &  &  &  &  &  &  &   &  \\
    % \hline
    ~\cite{sachidananda2023apter} & $2023$ & Heterogeneous Data-based  & TTPs from IDS/IPS and SIEM/EDR Alerts & TTP list & Sequential Classifier & $97.3$ & $96$ & $97$ & $97$ &   \\
    \hline
    ~\cite{xiao2024apt} & $2024$ & Threat reports & Node features of heterogeneous attributed graph schema  & ID encoding, Ordinal encoding, BERT encoding, and Node2vec encoding & Graph Neural Network & $-$ & $-$ & $-$ & $70.51$ &   \\
    \hline
    \end{tabularx}
\end{table*}
